Automated Feedback Generation for Introductory Programming Assignments

We present a new method for automatically providing feedback for introductory programming problems. In order to use this method, we need a reference implementation of the assignment, and an error model consisting of potential corrections to errors that students might make. Using this information, the system automatically derives minimal corrections to student's incorrect solutions, providing them with a quantifiable measure of exactly how incorrect a given solution was, as well as feedback about what they did wrong. We introduce a simple language for describing error models in terms of correction rules, and formally define a rule-directed translation strategy that reduces the problem of finding minimal corrections in an incorrect program to the problem of synthesizing a correct program from a sketch. We have evaluated our system on thousands of real student attempts obtained from 6.00 and 6.00x. Our results show that relatively simple error models can correct on average 65% of all incorrect submissions.

==> fuzz.tex <==
\section{Fuzzing Language}

language for specifying the fuzz model

two key constituents : context + rewrite transformations (fuzzes)
(similar to contextual semantics : set of contexts under which you are allowed to perform the reduction)

\subsection{Contexts}

Types of contexts:
- all
- loop -- initialization, conditional, increment
- array -- indexes
- methodcalls -- parameters --- number

\subsection{Rewrite Transformations}

define local transformations, such a way that we reach a fixpoint.

Kinds of transformations:
- statement transformation
- conditional transformation
- statement introduction transformation

We analyzed two different class of programming problems: simple loop
problems and recursion problems. 

\subsection{Fuzzing models}

\paragraph{loop problems}
\begin{enumerate}
\item array indices
$a[i] \rightarrow a[(i+1 | i-1 | i)]$
\item loop initialization
$i=k \rightarrow i = (k+1| k-1| 0)$
\item loop conditional
$i < k \rightarrow i (|< | > | \leq | \geq|) (|k+1|k-1|0|)$
\item loop increment
$i++ \rightarrow (|i++ | i-- | i=i+2| i=i-2|)$
\item conditionals
$== \rightarrow (|== | \geq | \leq | > | < | !=|)$
\item expression fuzzing
$expr + expr \rightarrow expr (|+|-|/|*|) expr$
\end{enumerate}

\paragraph{recursion problems}

\subsection{Concrete examples}

Rishabh will write the fuzz model (and provide examples that motivated
each construct in the fuzz model).

Sumit will formalize it.


==> oldsection2.tex <==






\begin{figure*}
\begin{tabular}{|c|c|}
\hline
\begin{minipage}{3.4in}
\begin{lstlisting}
using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = a;
    for (int i=1; i<=b.Length/2; i++){
      int temp = b[i];  
      b[i] = b[b.Length-i];  
      b[b.Length-i] = temp;  
    }
    return b;
  }
}
\end{lstlisting}
\end{minipage}

&
\begin{minipage}{3.4in}
\begin{verbatim}
Fix 1: Decrement index i by 1 in lines 7 and 8.

Fix 2: Decrement index b.Length-i by 1 in lines 8 
       and 9, Change for loop initiation i to 0.
\end{verbatim}
\end{minipage}
\\\hline
\end{tabular}
\caption{Two possible fixes to fix the student's attempt on the left}
\figlabel{multiple-fix}
\end{figure*}

Our tool is able to provide direct feedback to the student about what went wrong with their program. 



\subsection{Why another metric?}

The traditional way to grade programs have been using test cases. The
instructors typically have a collection of test cases and the student
is awarded marks corresponding to the fraction of test cases that the
student's implementation successfully passes. It is not a very
satisfactory way of grading because of two reasons. First, a program
which is very close to the correct solution may fail all the test
cases whereas a program which is far from the desired solution may
pass many test cases (a collection of if statements for each test
case). The second reason is that test cases do not translate to good
feedback, especially for beginner
students. Figure~\ref{fig-log-diverge} shows the log of a student's
attempt for array reverse problem taken from pex4fun where the
feedback that the system provided to the student was in the form of
passing and failing test cases. It is quite interesting to see that
during the course of solving the problem, the student first came close
to the correct solution but then diverged away by fixing the wrong
part of solution.

Another way to grade programs is to perform syntactic matching of
student's solution with the teacher's reference solution. This can
lead to providing better feedback if the student solutions are of a
similar kind to the reference solution.  This grading scheme is very
specific to the refrence solution and we can not expect students to
write algorithms in a way exactly similar to what teacher has in
mind. Figure~\ref{fig-different-attempts} shows some of the student
solutions for array reverse problems. The student solution in (a) uses
a while loop with two pointers front and back and the student solution
in (b) uses a for loop with half traversal over the array, whereas the
teacher soultion does a single complete traversal over the array using
a for loop.



\subsection{Semantic grading with feedback}

In this paper, we present a framework for performing atuomated
semantic grading of student programs. Our framework assigns a
quantitative score to a student solution based on a closeness
metric. The closeness metric defines how many changes we need to
perform in the student solution to make it semantically equivalent to
the teacher reference solution. Figure~\ref{fig-feedback} shows the
score and feedback provided by our framework to the student solution
on the left.

It is not always possible to understand automatically what the student
has in mind. For example Figure~\ref{fig-multiple-fix} shows two
possible fixes to the student solution on the left. The first fix
suggests to decrement the array index \texttt{i} by $1$ in lines $7$
and $8$ corresponding to the case of missing the first array
element. Another fix might be to initialize the loop variable
\texttt{i} to $0$ and decrement the array indices $\texttt{b.Length}
-\texttt{i}$ by $1$ in lines $8$ and $9$. Our framework optimizes on
the mininum number of changes that are needed to be performed, but
also supports for providing multiple fixes if the student feels the
provided feedback does not correspond to the intended algorithm.





\begin{figure*}
\begin{tabular}{|c|c|c|}
\hline
\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length-1; i<a.Length-1; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
  }
}

\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length-1; i<a.Length-1; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
  }
}

\end{verbatim}
\end{minipage}
\\
6:28:50 AM
&
6:32:01 AM
&
6:32:32 AM
\\\hline

\hline
\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<=a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      Console.Writeline(i);
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      Console.WriteLine(i);
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}
\\
6:33:19 AM
&
6:33:55 AM
&
6:34:06 AM
\\\hline

\hline
\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i=<a.Length; i--)
    {
      Console.WriteLine(i);
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length-1];
    int count = 0;
    for(int i=a.Length-1; i<a.Length-1; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}
\\
6:34:56 AM
&
6:36:24 AM
&
6:37:39 AM
\\\hline

\hline
\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i>0; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i>=0; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<i.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}
\\
6:38:11 AM
&
6:38:44 AM
&
6:39:33 AM
\\\hline

\hline
\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 1;
    for(int i=a.Length; i<a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length-1];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
  }
}
\end{verbatim}
\end{minipage}
\\
6:39:45 AM
&
6:40:27 AM
&
6:40:57 AM
\\\hline

\end{tabular}
\caption{Log of a student's attempts for array reverse problem}
\label{fig-log-diverge}
\end{figure*}




%% two column table example file
%% \begin{figure*}
%% \begin{tabular}{|c|c|}
%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length-1; i<a.Length-1; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }

%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:28:50 AM
%% &
%% 6:32:01 AM
%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length-1];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<=a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:32:32 AM
%% &
%% 6:33:19 AM

%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       Console.Writeline(i);
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       Console.WriteLine(i);
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }

%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:33:55 AM
%% &
%% 6:34:06 AM

%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i=<a.Length; i--)
%%     {
%%       Console.WriteLine(i);
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }

%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:34:56 AM
%% &
%% 6:36:24 AM

%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length-1];
%%     int count = 0;
%%     for(int i=a.Length-1; i<a.Length-1; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i>0; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:37:39 AM
%% &
%% 6:38:11 AM

%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i>=0; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<i.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:38:44 AM
%% &
%% 6:39:33 AM

%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 1;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:39:45 AM
%% &
%% 6:40:27 AM

%% \\\hline

%% \end{tabular}
%% \end{figure*}



==> related-work/abstract.tex <==
This paper presents a new method for automatically providing feedback for introductory programming assignments. In order to use this method, instructors provide a reference implementation of the assignment, and an error model consisting of potential corrections to errors that students might make. Using this information, the system automatically derives minimal corrections to incorrect student assignments, providing the students with direct feedback about exactly what they did wrong, as well as giving a quantifiable measure of exactly how incorrect a given solution was. 

The paper introduces a simple language for describing error models in terms of correction rules, and formally defines a rule-directed translation strategy that reduces the problem of finding minimal corrections to a problem of synthesizing a program from a sketch. The paper also describes an evaluation of our technique on over 1000 solution attempts by real beginner programmers. Our results show that relatively simple error models can correct on average over $70\%$
of submissions with small errors. We also show that the error models
generalize across different problems from the same category and
that our technique scales even for complex error models and larger programming assignments such as those found in AP level computer science final examinations. 



==> related-work/algorithm.tex <==
\section{Constraint-based Solving of $\implp$ programs}

In this section, we present the translation of $\implp$ programs into
constraints as \Sk{} programs and then present an algorithm to solve
these constraints to find an $\impl$ program in $\implp$ with the
least cost that is equivalent to a given teacher's reference solution.

\subsection{Translation of $\implp$ programs to \Sk{}}

We show the translation of some of the interesting $\implp$ constructs
to \Sk{} in \figref{fig-implp-trans}. The \Sk{} construct ?? (called
\emph{integer hole}) is a placeholder for a constant integer value,
which is filled up by the \Sk{} synthesizer while solving the
constraints to satisfy the given specification. In our translation, we
represent the guards (choices) as integer holes of 1-bit size where
the value $1$ corresponds to the guard being \t{true} and $0$
corresponding to the \t{false} case. The translation defines a global
integer variable \cost that is used to compute the number of
modifications in the original program to obtain the transformed
program.

A set-expression of the form $\saexpr = \{ \aexpr_0, \cdots, \aexpr_n,
\underline{\aexpr_b} \}$ is translated to a series of guarded
statements in \Sk{}: \sif(??)~\sreturn $\sem{\aexpr_b}$; \selse \{
\cost = \cost + 1; \sif(??) \sreturn $\sem{\aexpr_0}$; $\cdots$
\sif(??)~\sreturn $\sem{\aexpr_n}$;\}. We first let the synthesizer
select the base expression $\aexpr_b$. If the synthesizer selects this
choice during the solving phase, the value $\aexpr_b$ is returned
without incrementing the \cost variable as no transformation in the
original expression took place. If the synthesizer does not select the
base expression to meet the specification, the \cost variable is
incremented by $1$ as we are making a modification to the original
expression. The choice for other expressions in the set-expressions
$\aexpr_i$ is also encoded using guarded statements with 1-bit holes
as conditionals. The choices for array identifiers and function
identifiers are similarily expanded to a sequence of guarded
statements as shown in the figure.

The translation rules for $\sem{\saexpr_0[\saexpr_1] = \saexpr_2}$ and
$\sem{?\var = \saexpr}$ present the translation in cases when the
expressions are used on the left hand side of an assignment. In these
cases, the values are not returned but instead the left hand side is
expanded for all identifier expressions, which are then encoded as a
series of guarded statements in \Sk{}. The binary expressions and
statement choices are translated similarily as shown in the figure.


\begin{figure*}
\begin{eqnarray*}
& & \hspace*{-30mm}\saexpr=\{\aexpr_0,\cdots,\aexpr_n,\underline{\aexpr_b}\}, \sbexpr=\{\bexpr_0,\cdots,\bexpr_n,\underline{\bexpr_b}\}, \svar=\{\var_0,\cdots,\var_n,\underline{\var_b}\}, \op=\{\op_0, \cdots, \op_n,\underline{\op}\}\\
\sem{\{\aexpr_0, \cdots, \aexpr_n, \underline{\aexpr_b}\}} & = & \{\sif(??) ~\sreturn \sem{\aexpr_b}; \cost = \cost + 1; \sif(??)~\sreturn \sem{\aexpr_0}; \cdots \sif(??)~\sreturn \sem{\aexpr_n};\} \\
\sem{\{\bexpr_0, \cdots, \bexpr_n, \underline{\bexpr_b}\}} & = & \{\sif(??) ~\sreturn \sem{\bexpr_b}; \cost = \cost + 1; \cdots \sif(??)~\sreturn \sem{\bexpr_i}; \cdots\} \\
\sem{\saexpr_0[\saexpr_1]} & = & \{\sif(??) ~\sreturn \aexpr_{0b}[\sem{\saexpr_1}]; \cost = \cost + 1; \cdots \sif(??)~\sreturn \aexpr_{0i}[\sem{\saexpr_1}]; \cdots\}\\
\sem{?\var} & = & \{\cost = \cost + 1; \cdots \sif(??)~\sreturn \var_i; \cdots\}\\
\sem{\fs(\saexpr_1, \cdots, \saexpr_n} & = & \{\sif(??)~\sreturn f_b(\sem{\saexpr_1},\cdots,\sem{\saexpr_n}); \cost = \cost + 1; \cdots~\sif(??)~\sreturn~f_i(\sem{\saexpr_1}, \cdots, \sem{\saexpr_n});~\cdots\}\\
\sem{\saexpr_0[\saexpr_1] = \saexpr_2} & = & \{\sif(??)~\aexpr_{0b}[\sem{\saexpr_1}]=\sem{\saexpr_2}; \selse\{ \cost = \cost + 1; \cdots \elseif(??)~\aexpr_{0i}[\sem{\saexpr_1}]=\sem{\saexpr_2}; \elseif(??) \cdots\}\}\\
\sem{?\var = \saexpr} & = & \{\cost = \cost + 1; \sif(??)~\var_0=\sem{\saexpr};~ \cdots \elseif(??)~ \var_i=\sem{\saexpr}; \elseif(??) \cdots\}\\
\sem{\saexpr_0 ~ \saop ~ \saexpr_1} & = & \{\sif(??)~\sreturn ~\sem{\saexpr_0}~\op~\sem{\saexpr_1};~\cost = \cost + 1; \cdots \sif(??) ~\sreturn ~\sem{\saexpr_0}~\op_i~\sem{\saexpr_1}; \cdots\}\\
\sem{\svar := \saexpr} & = &  \{\sif(??)~ \var_b=\sem{\saexpr}; \selse \{ \sif(??) \var_0 = \sem{\saexpr}; \cdots ~\sif(??)~\var_i=\sem{\saexpr} ~ \elseif(??)\cdots \}\}\\
\sem{\{\sexpr_0, \cdots, \sexpr_n, \underline{\sexpr_b}\}} & = & \{\sif(??) ~\sreturn \sem{\sexpr_b}; \cost = \cost + 1; \cdots \sif(??)~\sreturn \sem{\sexpr_i};\cdots\} \\
\sem{\t{if} ~ \sbexpr ~ \t{then} ~ \ssexpr_0 ~ \t{else} ~ \ssexpr_1} & = & \{\sif(??)~ \t{if} ~ \bexpr_b ~ \t{then} ~ \sem{\sexpr_0} ~ \t{else} ~ \sem{\sexpr_1} else \{\cost = \cost + 1; \cdots ~ \elseif(??)~ \t{if}~\bexpr_i ~\t{then} ~\sem{\sexpr_0} ~\t{else} ~\sem{\sexpr_1} ~\elseif(??) ~ \cdots \} \}\\
\sem{\t{while} ~ \sbexpr ~ \t{do} ~ \ssexpr} & = & \{\sif(??) ~ \t{while} ~ \bexpr_b ~ \t{do} ~ \sem{\ssexpr}~ \selse \{\cost = \cost + 1; ~\cdots ~ \elseif(??)~ \t{while} ~ \bexpr_i ~ \t{do} ~ \sem{\ssexpr}~\elseif(??)  ~\cdots \}\}\\ 
\end{eqnarray*}
\caption{Some of the interesting translation rules for converting an $\implp$ program to a \Sk{} program}
\figlabel{fig-implp-trans}
\end{figure*}


\subsection{Computing the least-cost correct modification}

Once we have translated an $\implp$ program to a \Sk{} program, the
synthesizer now needs to solve these constraints to find a transformed
program with the least \cost such that it is semantically equivalent
to the teacher's reference solution. We first ask the synthesizer to
find a solution with an added assertion $(\t{assert}~\cost == 0)$,
i.e. the case in which the student program was correct in the first
place and did not require any modification. If the synthesizer can
find a solution, we exit the algorithm. Otherwise, the synthesizer
states that the constraints are unsatisfiable. We then increment the
$\cost$ variable by $1$ and ask the solver for a solution with an
assertion $(\t{assert}~\cost == 1)$, corresponding to the case in
which the student program requires a single modification to make it
semantically equivalent to the teacher's program. In this manner, we
repeatedly ask the synthesizer with increasing values of \cost until
we get a satisfiable constraint. We also put a bound on the maximum
value of \cost as $K$, such that if we can not find a solution for
$\t{assert}~\cost == K$ we report back that the student solution can
not be fixed using less than $K$ modifications. We set this bound to
$K=5$ for our case studies, which was adequate for all of the
benchmark examples. This algorithm calls the synthesizer $O(K)$ times,
but we can easily adapt the algorithm to perform a binary search on
$K$ instead of this linear search. In the case of binary search, we
would need to change the assertions on \cost to the form $(\t{assert}
~\cost \leq K)$. Since we kept $K=5$ for our experiments, we did not
implement the binary search algorithm as $K$ was small enough for
linear search to scale just as well.

\subsection{Computing Alternate Solutions}

It might happen that in some cases the solution that our tool computes
does not match the way in which the student was planning to solve the
problem. Consider the factorial function in \figref{fig-fact-mult}
which outputs $0$ instead of $1$ on $x = 0$. With the error model
consisting of adding the base case, the tool finds a fix to add the
base case for $x=0$. With the error model consisting of initialization
correction, the tool finds a solution where col is initialized to $1$
and the for loop iterator $i$ is initialized to $x$. Both the fixes
look perfectly viable and it is hard to prefer one over the other. To
cater to ssuch cases, our tool provides an option to ask for an
alternate solution if the suggested fix is not in sync with the
student's understanding. The tool asserts an additional assertion
corresponding to the negation of all unknown hole choices from the
previous solution to compute the next solution.
\begin{figure}
\begin{lstlisting}
using System;
public class Program {
  public static int Factorial(int x) {
    int col = x;
    for(int i = x-1 ; i >0; i--)
      col*= i;
    return col;
  }}
\end{lstlisting}
\caption{A student attempt for factorial function with two possible fixes: i) adding a base case for x=0, ii) initializing col to 1 and for loop initializer i to x}
\figlabel{fig-fact-mult}
\end{figure}

\subsection{Mapping \Sk{} solution to generate feedback}

Each transformation rule in the error model $\fm$ can be associated
with a feedback message, e.g. the array index transformation from
array-reverse error model $(\indF) \var[\aexpr] \rightarrow
\var[\aexpr+1]$ can be associated with a message such as ``the array
index needs to be incremented by 1'' or the base case transformation
($\baseF$) from factorial error model can be associated with ``the base
case of factorial method is missing''. After the \Sk{} synthesizer
finds a solution to the constraints, we map back the values of integer
holes to their correpsonding expression choices. These expression
choices are then mapped to natural language feedback using the
messages associated with the correpsonding correction rules, together
with the line numbers in the original code.



==> related-work/expr.tex <==
\section{Implementation and Experiments}
\label{sec-experiments}
The implementation of our framework consists of three phases: i)
Rewriting phase, ii) Solving phase and iii) Feedback generation
phase. The Rewriting phase parses and rewrites a student solution
(written in \csharp) to a program in $\fuzzc$ language ($\implp$
variant of \csharp). We use Microsoft's Roslyn compiler
framework\footnote{Microsoft Roslyn Framework
  http://msdn.microsoft.com/en-us/roslyn} for performing the rewrites
based on a set of correction rules. The Solving phase consists of
translating the $\fuzzc$ program into a \Sk{} program and then solving
the sketch program to compute minimal modifications to the original
program for making it semantically equivalent to the teacher
solution. We use the \Sk{} solver for efficiently solving these
$\exists\forall$ constraints. Finally, the Feedback phase maps the
modifications in the student solution to their corresponding
explanations in natural language for generating the feedback.

\subsection{Benchmarks}

We collected logs of $5$ loops-over-arrays problems: \t{array
  reverse}, \t{palindrome}, \t{is array sorted}, \t{array max} and
\t{array sort} as well as a recursion problem \t{factorial} from the
\pexfun website. Our selection criteria for selecting these problems
was to select the problems which were suitable for beginner
programmers and for which there was a clear description on what the
users were supposed to program. Typically problems on \pexfun website
are puzzle problems and users figure out the specification via failing
input-output test cases; we wanted to avoid such problems as it is
hard to evaluate the fixes on such problems since most of the time the
fault will be present because of the unknown spec. The \t{fibonacci}
problem on the website was a tricky variant of the traditional case,
without any spec, so we did not include it in our benchmark set. From
this set of thousands of attempts we removed the following attempts that:
\begin{itemize}
\item had compilation errors
\item used library methods like \t{Array.Sort}, \t{Array.Reverse} etc.
\item used generics like \t{List<int>}
\item no loops in for loops-over-array problems
\item very far from desired solution (e.g. adding array elements for array reverse problem, printing a constant inside loop)
\end{itemize}

We also created a few descriptive problems adapted from an AP high
school computer science final examination: \t{friday restaurant rush}
and \t{longest dice throw} problems. Each one of these problems
involves computing maximum contiguous subset sum of the input array.

\subsection{Repetitive mistakes}
We first investigate our hypothesis that many students make similar
mistakes when solving a given problem. For each benchmark set, we
first ran the student solutions without any modifications to obtain
the set of buggy solutions. From this set, we picked the first buggy
solution that can be fixed using our correction langauge and then we
added the corresponding correction rule to the error model. We then
re-ran the benchmarks to get another (smaller) set of failing
solutions. We kept repeating this step of picking the first buggy
solution and enchancing the erro model until we acheived the maximum
possible coverage of fixing the buggy solutions.

The results of this experiment are shown in
Figure~\ref{fuzzmodelcoverage}. The horizontal axis shows different
error models $\fm$ in monotonically increasing order of number of
correction rules, such that $\fm_i \subset {\fm_j}_{ \forall i <
  j}$. The vertical axis shows the number of buggy solutions that were
fixed using these error models. For the array reverse problem, the
error models $\fm_1 = \{\initF$\} fixed $21$ solutions, $\fm_2 = \fm_1
\cup \{\condF$\} fixed $107$ solutions, $\fm_3 = \fm_2 \cup \{\indF\}$
fixed $235$ solutions, $\fm_4 = \fm_3 \cup \{\retF\}$ fixed $252$
solutions and $\fm_5 = \fm_4 \cup \{\incF\}$ fixed $254$ solutions. We
had to look at only $5$ buggy solutions and around $10$-$15$
out-of-scope solutions to correct around $250$ buggy solutions. We
obtained similar results for other benchmarks as well. These results
support our hypothesis that students make similar mistakes while
solving a given problem, and hence we can correct a large number of
buggy attempts by looking at only a small number of buggy solutions.

\begin{figure}
\begin{center}
\includegraphics[scale=0.30]{figures/graph1.pdf}
\caption{The fraction of buggy solutions fixed with varying fuzzmodels $\fm$}
\end{center}
\label{fuzzmodelcoverage}
\end{figure}

\subsection{Generalization of Error Models}

We next investigate the hypothesis that error models generalize well
accross different problems of same category. For performing this
experiment, we took the error model for the array-reverse problem and
used it as error model for other problems in the loops-over-arrays
category. The results of this experiment are shown in
Figure~\ref{generalizefuzzmodel}. As we can see from the figure, the
error model generalizes well for some problems and not so well for the
others. But teachers can use it as a good starting point for new
problems in the same category. This error model can then be specialized
by adding problem specific fuzz rules to achieve greater fix coverage.

\begin{figure}
\begin{center}
\includegraphics[scale=0.32]{figures/graph3.pdf}
\caption{Performance of array reverse fuzz model on other loop problems$\fm$}
\label{generalizefuzzmodel}
\end{center}
\end{figure}


\subsection{Performance}

We compare the performance of our tool on varying complexity of error
models in Figure~\ref{figtradeoff}. We would expect that the tool will
take more time to compute the fixes with the increase in complexity of
error models (as the size of the search-space of corrections
increases). However, from the figure we can see that the running time
is not increasing monotonically with the increase in error model
complexity. The reason for this phenomenon is that even though the
search-space of corrections is becoming bigger, there are also newer
solutions available for the constraint solver which were not available
before in a less complex error model.

\begin{figure}
\begin{center}
\includegraphics[scale=0.32]{figures/graph2.pdf}
\caption{Average time (in s) to fix buggy problems$\fm$}
\label{figtradeoff}
\end{center}
\end{figure}


\subsection{Expressiveness of Correction language}

Table~\ref{tabExpressivity} presents the fraction of buggy solutions
that our framework was able fix for the benchmark problems. Our error
models were able to fix majority of small errors. Some fixes required
reordering of statements and introducing statements with complicated
logic which our tool currently does not support. The table also shows
the result on the Friday rush problem, we present its result to show
that our approach scales to such problems as well.
\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Benchmark} & \textbf{Total} & \textbf{Fixed} & \textbf{Changes} & \textbf{Time(s)}\\
\hline
Array reverse & 305 & 254 & 1.73& 2.69\\
\hline
String palindrome & 86 & 64 & 1.28& 3.52\\
\hline
Array maximum & 99 & 68 & 1.25 & 7.47\\
\hline
Is Array increasing & 51 & 38 & 1.72 & 3.56 \\
\hline
Array sort & 74 & 35 & 1.17 & 32.46\\
\hline
Factorial & 70& 40& 1.25& 4.99 \\
\hline
Friday rush & 17& 4& 1 & 12.42 \\
\hline
\end{tabular}
\end{center}
\label{tabExpressivity}
\caption{The percentage of benchmarks that were fixed with average number of changes and average time taken per problem}
\end{table}

\subsection{Quality of fixes}

To evaluate the quality of the fixes suggested by the framework, we
manually investigated the student s next attempts on the same
problem. In the cases where student had not given up, we found that
the fixes suggested by our framework matched student's correction in
most cases.



==> related-work/fuzz.tex <==
\section{Fuzzing Language}

language for specifying the fuzz model

two key constituents : context + rewrite transformations (fuzzes)
(similar to contextual semantics : set of contexts under which you are allowed to perform the reduction)

\subsection{Contexts}

Types of contexts:
- all
- loop -- initialization, conditional, increment
- array -- indexes
- methodcalls -- parameters --- number

\subsection{Rewrite Transformations}

define local transformations, such a way that we reach a fixpoint.

Kinds of transformations:
- statement transformation
- conditional transformation
- statement introduction transformation

We analyzed two different class of programming problems: simple loop
problems and recursion problems. 

\subsection{Fuzzing models}

\paragraph{loop problems}
\begin{enumerate}
\item array indices
$a[i] \rightarrow a[(i+1 | i-1 | i)]$
\item loop initialization
$i=k \rightarrow i = (k+1| k-1| 0)$
\item loop conditional
$i < k \rightarrow i (|< | > | \leq | \geq|) (|k+1|k-1|0|)$
\item loop increment
$i++ \rightarrow (|i++ | i-- | i=i+2| i=i-2|)$
\item conditionals
$== \rightarrow (|== | \geq | \leq | > | < | !=|)$
\item expression fuzzing
$expr + expr \rightarrow expr (|+|-|/|*|) expr$
\end{enumerate}

\paragraph{recursion problems}

\subsection{Concrete examples}

Rishabh will write the fuzz model (and provide examples that motivated
each construct in the fuzz model).

Sumit will formalize it.


==> related-work/fuzzlanguage.tex <==
\section{Correction Language}
\seclabel{fuzzlanguage} In this section, we formally define our
framework in terms of a simple imperative language $\impl$. We first
define a language $\implp$ that we use to represent a sets
of programs in $\impl$ succinctly. We then define an error model as a set of correction rules $\fm$ that rewrite a program in $\impl$ to one in
$\implp$. Finally, we define a program in $\implp$ to be a set of
weighted programs in $\impl$ such that the weight quantifies the
number of modifications made in the original program to obtain the
transformed program.

\subsection{$\impl$ and $\implp$ languages}

The syntax for our simple imperative language $\impl$ extended with
function calls is shown in Figure~\ref{fig-lang-table}(a). The
semantics for $\impl$ language is straightforward and can be found in
~\cite{WinskelBook}. Figure~\ref{fig-lang-table}(b) shows the syntax
for the language $\implp$. The purpose of $\implp$ language is to
represent a large collection of programs in $\impl$ succinctly. The
$\implp$ language consists of set-expressions ($\saexpr$, $\sbexpr$
and $\ssexpr$) that represent a set of expressions from $\impl$. In
addition, it contains a special construct $?\var$ which denotes the
set of all variables of type $\var$ which are in scope at the
corresponding program location. We found this construct to be
extremely useful and convenient for correcting student programs in our
case studies as described in Section~\ref{sec-experiments}.

\begin{figure*}[!htpb]
\begin{tabular}{c|c}
\begin{minipage}{3.5in}
\begin{eqnarray*}
\mbox{Arithmetic Expression } \aexpr & \bnfas & \intN  ~ \bnfalt ~ \var ~ \bnfalt ~ \aexpr[\aexpr] ~ \bnfalt ~ \aexpr_0 ~ \aop ~ \aexpr_1\\
& \bnfalt & \fvar(\aexpr_0, \cdots, \aexpr_n)\\
\mbox{Arithmetic Operator } \aop & \bnfas & + ~ \bnfalt ~ - ~ \bnfalt ~ \times ~ \bnfalt ~/\\
\mbox{Boolean Expression } \bexpr & \bnfas & \lnot ~ \bexpr ~ \bnfalt ~ \aexpr_0 ~ \bop ~ \aexpr_1 ~ \bnfalt ~\bexpr_0 ~ \cop ~ \bexpr_1\\
\mbox{Boolean Operator } \bop & \bnfas & == ~ \bnfalt ~ < ~ \bnfalt  ~ > ~ \bnfalt~ \leq ~ \bnfalt \geq\\
\mbox{Boolean Conjunction } \cop & \bnfas & \land ~ \bnfalt ~ \lor\\
\mbox{Statement Expression } \sexpr & \bnfas & \var := \aexpr; ~ \bnfalt ~ \sexpr_0;\sexpr_1 ~ \bnfalt ~ \t{while} ~ \bexpr ~ \t{do} ~ \sexpr\\
 &\bnfalt & \t{if} ~ \bexpr ~ \t{then} ~ \sexpr_0 ~ \t{else} ~ \sexpr_1\\
& \bnfalt & \t{return} ~ \aexpr\\
\mbox{Program } \prog & \bnfas & \t{method} ~ f(\aexpr_1, \cdots, \aexpr_n) ~\sexpr
\end{eqnarray*}
\end{minipage}
&
\begin{minipage}{3.5in}
\begin{eqnarray*}
\mbox{Arithmetic Expressions } \saexpr & \bnfas & \ldots  ~ \bnfalt \choosevar\var ~ \bnfalt \{\aexpr_0, \cdots, \aexpr_n \}\\
\mbox{Boolean Expressions } \sbexpr & \bnfas & \ldots ~ \bnfalt \{\bexpr_0, \cdots, \bexpr_n \}\\
\mbox{Statement Expressions } \ssexpr & \bnfas & \ldots ~ \bnfalt \{\sexpr_0, \cdots, \sexpr_n\}
\end{eqnarray*}
\end{minipage}\\\\
(a)~$\impl$ & (b)~$\implp$ \\
\end{tabular}
\caption{The syntax for (a) $\impl$ and (b) $\implp$ languages}
\label{fig-lang-table}
\end{figure*}

\subsection{Error model $\fm$}

An error model $\fm$ consists of a set of correction rules which are
used to rewrite a program in $\impl$ to a set of programs that are
represented as a program in $\implp$. A {\em correction rule} $\fm_i :
\impl \rightarrow \implp$ is written in the form $L \rightarrow R$,
where $L$ and $R$ can denote a \emph{program element} $\wexpr$ in
$\impl$ and $\implp$ respectively. A program element can either be a
term, an expression, a statement or the program itself. One
restriction our framework enforces in defining these rules is that
only the left hand side $L$ of the rule can have free variables and
the variables in the right hand side $R$ can only refer to the
variables present in $L$. The error models for the array-reverse
problem and factorial problem are shown in
Figure~\ref{fig-fuzz-array-reverse} and \figref{fig-error-model-fact}
respectively.
\begin{figure}
\begin{eqnarray*}
\mbox{\indF} ~~\var[\aexpr] & \rightarrow & \var[\{\aexpr+1, \aexpr-1,\aexpr-?\aexpr,\var.\t{Length}-\aexpr-1\}]\\ 
\mbox{\initF} ~~\var=\intN & \rightarrow & \var = \{n+1, n-1, 0\}\\ 
\mbox{\condF} ~~ \bexpr_0 ~ \bop ~  \aexpr_0 ~ & \rightarrow & \bexpr_0\dash ~\sbop ~\{\aexpr_0+1, \aexpr_0-1, 0, 1, ?\aexpr_0 \} \\ 
& & \hspace*{-12mm}\mbox{where } \sbop = \{<, >, \leq, \geq, ==, \neq\}\\ 
\mbox{\incF} ~~\var++ & \rightarrow & \{++\var, --\var, \var--\}\\ 
\mbox{\retF} ~~\t{return}~\var & \rightarrow & \t{return} ~?\var\\ 
%\mbox{\arithF} ~~\aexpr & \rightarrow & \{\aexpr+1, \aexpr - 1, 0, ?\aexpr-\aexpr-1\}\\ 
\end{eqnarray*}
\caption{The error model $\fm$ for array reverse problem}
\label{fig-fuzz-array-reverse}
\end{figure}

\begin{figure}
\begin{eqnarray*}
\mbox{\funcF }~~ f(\aexpr_1,\cdots,\aexpr_n) & \rightarrow  & f(\saexpr_1,\cdots,\saexpr_n)\\
& & \hspace*{-23mm}\mbox{where } \saexpr_i = \{\aexpr_i + 1, \aexpr_i - 1\}\\ 
\mbox{\basecF }~~ \t{method}~ \t{fact}(\aexpr)~ \sexpr & \rightarrow & \t{method}~ \t{fact}(\aexpr) ~ \sexpr_{base};\sexpr\\
& & \hspace*{-23mm}\mbox{where } \sexpr_{base} = ~\sif ~(\aexpr == 0)~ \t{return} ~1;\\ 
\mbox{\initF} ~~\var=\intN & \rightarrow & \var = \{n+1, n-1, 1, 0\}\\ 
\mbox{\condF }~~ \bexpr_0 ~ \bop ~  \aexpr_0 ~ & \rightarrow & \bexpr_0\dash ~ \sbop ~ \{\aexpr_0 + 1,\aexpr_0 - 1, 0 \} \\ 
& & \hspace*{-12mm}\mbox{where } \sbop = \{<, >, \leq, \geq, ==, \neq\}\\ 
\end{eqnarray*}
\caption{The error model $\fm$ for factorial problem}
\figlabel{fig-error-model-fact}
\end{figure}

The semantics of application of correction rules (\transExpr) is
better understood with the help of an example first. Let us consider
an error model $\fm$ consisting of the following two correction rules:
\begin{eqnarray*}
\mbox{$\fm_1 : $} ~~ \var[\aexpr] & \rightarrow & \var'[\aexpr+1, 0]\\
\mbox{$\fm_2 : $} ~~ \sreturn \var & \rightarrow & \sreturn ?\var\\
\end{eqnarray*}

This error model $\fm$ is translated to a transformation function
\transExpr~ as

\begin{eqnarray*}
\transExpr(\fm: \impl \rightarrow \implp, \wexpr: \impl) : \implp & = & \\
& & \hspace*{-62mm} \t{let} ~ \wexpr_0 = \wexpr[t\rightarrow\transExpr(\fm,t)] ~ \t{in}\\
& & \hspace*{-58mm} \t{let} ~ \wexpr_1 = \matchE ~ \wexpr ~\t{with} ~\var_0[\aexpr_0] \rightarrow \transExpr(\fm,\var_0)[\{\aexpr_0+1, 0\}] ~ \t{in}\\
& & \hspace*{-54mm} \t{let} ~  \wexpr_2 = \matchE ~\wexpr ~\t{with} ~\sreturn ~\var_0 \rightarrow \sreturn ~?\var_0 ~ \t{in}\\
& & \hspace*{-44mm} \wexpr_0 \cup \wexpr_1 \cup \wexpr_2
\end{eqnarray*}

A program element $\wexpr$ is first traveresed in the default way,
i.e. no rewriting happens at this level of the abstract syntax tree
and the \transExpr method is called recursively on all of its
sub-terms $t$. For each correction rule $\fm_i$ in the error model, we
have a \matchE expression that matches the term $\wexpr$ with the left
hand side of the rule $L_i$ with appropriate unification of the free
variables in $L_i$. If the match succeeds, it is transformed to a term
as defined by the right hand side $R_i$ of the rule after applying the
$\transExpr$ method recursively on each one of its primed sub-terms
$t\dash$. Finally, the method \transExpr returns the union of all the
transformed terms $\wexpr_i$. The general semantics for \transExpr
method is shown in Figure~\ref{transsemantics}. There are two
interesting things to note here:


\begin{figure}
\begin{eqnarray*}
\transExpr(\fm: \impl \rightarrow \implp, \wexpr: \impl) : \implp & =
& \\ & & \hspace*{-55mm} \t{let} ~ \wexpr_0 =
\wexpr[t\rightarrow\transExpr(\fm,t)] ~\t{in}\\ & & \hspace*{-50mm}
\t{let} ~ \wexpr_i = \matchE ~ \wexpr ~\t{with} ~L_i ~ \rightarrow ~
R_i[t'~\rightarrow~\transExpr(\fm,t)] ~ \t{in}\\ & & \hspace*{-45mm}
\bigcup_{0\leq i\leq n} \wexpr_i
\end{eqnarray*}
\caption{$\transExpr$ method for applying correction rules in $\fm$}
\label{transsemantics}
\end{figure}

%interesting cases that
%arise when performing these transformations:

\begin{itemize}
{\item Nested Rewritings :} Once a correction rule is applied to
transform a term $L$ to $R$, we sometimes need to apply a correction
on a sub-term of $R$ but not on all of its sub-terms.  For example, we
may want to avoid rewriting the sub-terms which have already been
rewritten by the correction rule. Our framework facilitates making
such distinction between the sub-terms for nested transformations
using the $\prime$ (prime) operator. A sub-term in $R$ that is tagged
with the prime operator is visited for applying further rewriting on
it (using the $\transExpr$ method recursively on its primed sub-terms
$t\dash$), whereas the remaining sub-terms without the prime operator
are not visited for rewriting any further. For example, consider the
conditional correction rule from array-reverse :
$(\condF)$~~$\bexpr_0$ $\bop$ $\aexpr_0$ $\rightarrow$ $\bexpr_0\dash$
$\sbop$ $\{\aexpr_0+1, \aexpr_0-1, 0, 1, ?\aexpr_0 \}$. Here we have
sub-expression $\bexpr_0$ in $R$ that is tagged with the prime
operator whereas the sub-expression $\aexpr_0$ is not. To perform this
rewriting on expression $\bexpr_0~ \bop ~\aexpr_0$, $\aexpr_0$ is
rewritten to the set-expression $\{\aexpr_0+1, \aexpr_0-1, 0, 1,
?\aexpr_0 \}$ whereas $\bexpr_0$ is further rewritten recursively.

\item {Ambiguous Rewritings :} When performing these rewritings, it
  may happen that there are multiple correction rules that pattern
  match the program element \wexpr in the abstract syntax tree. For
  example, there can be two correction rules for rewriting array
  accesses, one that corrects the indices $\var[\aexpr] \rightarrow
  \var[\{\aexpr+1, \aexpr - 1, 0\}]$ and the other that corrects the
  array identifier $\var[\aexpr] \rightarrow ?\var[\aexpr]$. After
  applying one of these rules to an expression $\var[\aexpr]$, we
  cannot apply the other rule to the same expression. In such
  ambiguous cases, $\transExpr$ creates a separate copy of the
  transformed abstract syntax tree ($\wexpr_i$) for each ambigous
  choice and then takes the set union of all such abstract syntax
  trees to obtain the transformed expression. This semantics of
  handling ambiguity in correction rules also matches naturally with
  the intent of the teacher. If the teacher wished to perform both the
  corrections together on array accesses, she could have provided a
  combined correction rule such as $\var[\expr] \rightarrow
  ?\var[\{\aexpr+1, \aexpr-1, 0\}]$.
\end{itemize}

\begin{definition} Well-formed Correction Rules : A correction rule $\fm_i : L \rightarrow R$ is defined to be well-formed if all tagged sub-terms $t\dash$ of $R$ have a smaller size syntax tree than that of $L$.
\end{definition}

The correction rule $\fm_1: \var[\aexpr] \rightarrow
\var[(\var[\aexpr])\dash]$ is not a well-formed correction rule as the
size of sub-term (\var[\aexpr]) in $R$ is the same as that of the left
side $L$. On the other hand the correction rule $\fm_2: \var[\aexpr] \rightarrow \var[\var\dash[\aexpr\dash]]$ is a well-formed correction rule.

\begin{definition} Well-formed Error Model : An error model $\fm$ is defined to be well-formed if all its constituent correction rules $\fm_i \in \fm$ are well-formed.
\end{definition} 

\begin{theorem}
The method $\transExpr$ with a well-formed error model $\fm$ always terminates. \end{theorem}
\begin{proof}
We prove the theorem inductively on the size of the syntax trees
produced on the right hand side of the correction rules. Application
of each correction rule is guaranteed to reduce the size of the syntax
tree and hence it terminates in finite number of rewrite applications.
\end{proof}

\subsection{$\implp$ programs as weighted sets}

A program in $\implp$ represents a set of programs in $\impl$ and is
obtained by rewriting a program in $\impl$ using the correction rules
$\fm$. Each transformed program is associated with a cost metric $c$
which encodes the distance of the transformed program from the
original program. The motivation behind this cost metric is to
quantify the number of changes that are performed in the original
program to obtain the transformed program. With this quantification,
we can now solve for questions like ``give me the minimum distance
transformed program that satisfies some
condition''. Figure~\ref{fig-implp-impl} shows the algorithm to
compute the costs of the transformed programs recursively. For
terminals in $\impl$ such as integers ($\intN$) and operators ($\op$),
we associate a cost of $0$ if the terminal in the transformed term is
the same terminal as that in the original term (the original terminal
is denoted by an underline below it). If the transformed term contains
some other terminal that is not equal to the terminal in the original
term, we associate a cost of $1$ with such a transformed term. For the
set of expressions, we associate a cost of $c$ if the expression in
the transformed program $\aexpr$ is the same as that of the original
expression or a cost of $c$+1 otherwise, where $c$ denotes the cost
associated with the transformation of expression $\aexpr$. The costs
for other constructs in the language are similarily computed
recursively as shown in the figure.

\noindent{\bf Extension of cost metric:} We have presented a
simplified cost metric of associating cost $1$ with each
correction. The cost framework can easily be extended to account for
different costs associated with different correctionss. This is
usually the case when some mistakes that students make should be
penalized more than the ones which are minor. For example, forgetting
to add a base case in a recursive formula might deserve more penalty
than mistaking the conditional operator $<$ instead of
$\leq$. The function of adding costs of sub-expressions can also
be generalized to other functions to cater for different grading schemes.

%% \begin{figure}
%% \hspace*{-3mm}\begin{program}[style=tt,number=true]
%% \stab{1mm}\hspace*{-2mm}\underline{$\transExpr$}($\expr$: $\impl$, $\fm$: $\impl \rightarrow \implp$)\nonumber 
%% if $\matchE(\expr, L_1)$ then $\exprs = \exprs \cup \transSubExpr(R_1)$
%% if $\matchE(\expr, L_2)$ then $\exprs = \exprs \cup \transSubExpr(R_2)$
%% $\vdots$
%% $\exprs = \exprs \cup \{\expr\}$
%% $\t{return}~\exprs$
%% \end{program}
%% \end{figure}




%% \begin{figure*}
%% \begin{tabular}{c|c}
%% \begin{minipage}{3.5in}
%% \begin{eqnarray*}
%% \mbox{Arithmetic Expression } \aexpr & \bnfas & \intN \\
%%                          & \bnfalt & \var \\
%%                          & \bnfalt & \var[a]\\
%%                          & \bnfalt & \aexpr_0 ~ \aop ~ \aexpr_1\\
%%                           & \bnfalt & f(\aexpr_1, \cdots, \aexpr_n)\\
%% \mbox{Arithmetic Operator } \aop & \bnfas & + ~ \bnfalt ~ - ~ \bnfalt ~ \times\\
%% \mbox{Boolean Expression } \bexpr & \bnfas & \lnot ~ \bexpr\\
%%                           & \bnfalt & \aexpr_0 ~ \bop ~ \aexpr_1 \\
%%                           & \bnfalt & \bexpr_0 ~ \cop  ~ \bexpr_1\\
%% \mbox{Boolean Operator } \bop & \bnfas & == ~ \bnfalt ~ < ~ \bnfalt  ~ > ~ \bnfalt~ \leq ~ \bnfalt \geq\\
%% \mbox{Boolean Conjunction } \cop & \bnfas & \land ~ \bnfalt ~ \lor\\
%% \mbox{Statement Expression } \sexpr & \bnfas & \var := \aexpr \\
%%                            & \bnfalt & \sexpr_0;\sexpr_1\\
%%                            & \bnfalt & \t{if} ~ \bexpr ~ \t{then} ~ \sexpr_0 ~ \t{else} ~ \sexpr_1\\
%%                            & \bnfalt & \t{while} ~ \bexpr ~ \t{do} ~ \sexpr
%% \end{eqnarray*}
%% \end{minipage}
%% &
%% \begin{minipage}{3.5in}
%% \begin{eqnarray*}
%% \mbox{Arithmetic Expressions } \saexpr & \bnfas & \sintN \\
%%                          & \bnfalt & \svar \\
%%                          & \bnfalt & \svar[\saexpr]\\
%%                          & \bnfalt & \saexpr_0 ~ \saop ~ \saexpr_1\\
%%                           & \bnfalt & \tilde{f}(\saexpr_1, \cdots, \saexpr_n)\\
%% \mbox{Boolean Expressions } \sbexpr & \bnfas & \lnot ~ \sbexpr\\
%%                           & \bnfalt & \saexpr_0 ~ \sbop ~ \saexpr_1 \\
%%                           & \bnfalt & \sbexpr_0 ~ \scop  ~ \sbexpr_1\\
%% \mbox{Statement Expressions } \ssexpr & \bnfas & \svar := \saexpr \\
%%                            & \bnfalt & \ssexpr_0;\ssexpr_1\\
%%                            & \bnfalt & \t{if} ~ \sbexpr ~ \t{then} ~ \ssexpr_0 ~ \t{else} ~ \ssexpr_1\\
%%                            & \bnfalt & \t{while} ~ \sbexpr ~ \t{do} ~ \ssexpr
%% \end{eqnarray*}
%% \end{minipage} \\\\
%% $\impl$ & $\implp$ \\
%% \end{tabular}
%% \caption{The syntax for $\impl$ and $\implp$ languages}
%% \label{fig-lang-table}
%% \end{figure*}

\begin{figure*}
\begin{eqnarray*}
\sem{\{\intN\}} & = & \{(n,0)\}\\
\sem{\{\var\}} & = & \{(\var,0)\}\\
\sem{\{\op_0, \cdots, \op_k, \underline{\op}\}} & = & \{(\op_i,1) \where 0 \leq i \leq k\} \cup \{(\op, 0)\}\\
\sem{\{\aexpr_0, \cdots, \aexpr_n, \underline{\aexpr_b}\}} & = & \{(\aexpr,~c+1) \where (\aexpr,c)\in\sem{\aexpr_i} \} \cup \sem{\aexpr_b}\\
\sem{\{\bexpr_0, \cdots, \bexpr_n, \underline{\bexpr_b}\}} & = & \{(\bexpr,~c+1) \where (\bexpr,c)\in\sem{\bexpr_i} \} \cup \sem{\bexpr_b}\\
\sem{\{\sexpr_0, \cdots, \sexpr_n, \underline{\sexpr_b}\}} & = & \{(\sexpr,~c+1) \where (\sexpr,c)\in\sem{\sexpr_i} \} \cup \sem{\sexpr_b}\\
\sem{\saexpr_0[\saexpr_1]} & = & \{(\aexpr_0[\aexpr_1],~c_0+c_1) \where (\aexpr_0,c_0)\in \sem{\saexpr_0}, (\aexpr_1,c_1) \in \sem{\saexpr_1} \}\\
\sem{?\var} & = & \{(\var_1,1) \where \var_1 \in \varinscope(\var), \var_1 \neq \var \} ~ \cup \sem{\var}\\
\sem{ \fs(\saexpr_1, \cdots, \saexpr_n} & = & \{(f(\aexpr_1,\cdots,\aexpr_n),~c_f+c_1\cdots+c_n) \where (f,c_f)\in\sem{\fs}, (\aexpr_i,c_i) \in \sem{\saexpr_i} \}\\
\sem{\saexpr_0 ~ \saop ~ \saexpr_1} & = & \{(\aexpr_0 ~ \aop ~ \aexpr_1, ~c_0+c_a+c_1) \where (\aexpr_0,c_0)\in\sem{\saexpr_0}, (\aop,c_a)\in\sem{\saop}, (\aexpr_1,c_1)\in\sem{\saexpr_1} \}\\
\sem{\saexpr_0 ~ \sbop ~ \saexpr_1} & = & \{(\aexpr_0 ~ \bop ~ \aexpr_1, ~c_0+c_b+c_1) \where (\aexpr_0,c_0)\in\sem{\saexpr_0}, (\bop,c_b)\in\sem{\sbop}, (\aexpr_1,c_1)\in\sem{\saexpr_1} \}\\
\sem{\sbexpr_0 ~ \scop ~ \sbexpr_1} & = & \{(\bexpr_0 ~ \cop ~ \bexpr_1, ~c_0+c_c+c_1) \where (\bexpr_0,c_0)\in\sem{\sbexpr_0}, (\cop,c_c)\in\sem{\scop}, (\bexpr_1,c_1)\in\sem{\sbexpr_1} \}\\
\sem{\svar := \saexpr} & = &  \{(\var := \aexpr, ~c_0 + c_1) \where (\var,c_0) \in \sem{\svar}, (\aexpr,c_1) \in \sem{\saexpr}\}\\
\sem{\ssexpr_0;\ssexpr_1} & = & \{ (\sexpr_0;\sexpr_1, ~c_0+c_1) \where (\sexpr_0,c_0) \in \sem{\ssexpr_0}, (\sexpr_1,c_1) \in \sem{\ssexpr_1}\}\\
\sem{\t{if} ~ \sbexpr ~ \t{then} ~ \ssexpr_0 ~ \t{else} ~ \ssexpr_1} & = & \{(\t{if} ~ \bexpr ~ \t{then} ~ \sexpr_0 ~ \t{else} ~ \sexpr_1, ~c_b+c_0+c_1) \where (\bexpr,c_b) \in \sem{\sbexpr}, (\sexpr_0,c_0) \in \sem{\ssexpr_0}, (\sexpr_1,c_1) \in \sem{\ssexpr_1}\}\\
\sem{\t{while} ~ \sbexpr ~ \t{do} ~ \ssexpr} & = & \{(\t{while} ~ \bexpr ~ \t{do} ~ \sexpr, ~ c_b + c_s) \where (\bexpr,c_b) \in \sem{\sbexpr}, (\sexpr,c_s) \in \sem{\ssexpr}\}\\ 
\sem{\t{return} ~ \saexpr} & = & \{(\t{return} ~ \aexpr, ~ c) \where (\aexpr,c) \in \sem{\aexpr}\}\\ 
\end{eqnarray*}
\caption{The translation of a program in $\implp$ to a set of programs in $\impl$, each associated with a cost $c$}
\figlabel{fig-implp-cost}
\end{figure*}

%% \begin{figure*}
%% \begin{center}
%%   \begin{tabular}{c c c}
%% \inference{t_1 \rightarrow_R t_2}{t_1 \rightarrow^{*}_R t_2}
%% &
%% \inference{t_1 \rightarrow^{*}_R t_3 & t_3 \rightarrow^{*}_R t_2}{t_1 \rightarrow^{*}_R t_2}
%% &
%% \inference{t_1 \rightarrow^{*}_R t'_1 ~~~~\cdots ~~~~ t_n \rightarrow^{*}_R t'_n}{c(t_1,\cdots,t_n) \rightarrow^{*}_R c(t'_1, \cdots, t'_n)}

%% \end{tabular}
%% \end{center}
%% \caption{Semantics for term rewriting rules}
%% \end{figure*}

%% \begin{figure*}
%% \begin{center}
%% \begin{tabular}{c c c}
%% \inference{t_1 \rightarrow^{i}_R t'_1 ~~~~\cdots ~~~~ t_n \rightarrow^{i}_R t'_n ~~~~ c(t'_1,\cdots,t'_n) \rightarrow^{r}_R t}{c(t_1,\cdots,t_n) \rightarrow^{i}_R t}
%% &
%% \inference{t_1 \rightarrow_R t_2 ~~~~ t_2 \rightarrow^{i}_R t_3}{t_1 \rightarrow^{r}_R t_3}
%% &
%% \inference{\lnot \exists t_2 : t_1 \rightarrow_R t_2 }{t_1 \rightarrow^{r}_R t_1}
%% \end{tabular}
%% \end{center}
%% \caption{Semantics for Innermost term rewriting strategy}
%% \end{figure*}

%% \begin{figure*}
%% \begin{tabular}{c|c}
%% \begin{minipage}{3.5in}
%% \begin{eqnarray*}
%% \mbox{Array Indexes } \var[\aexpr] & \rightarrow & \var[\{\aexpr+1, \aexpr-1,\aexpr \}]\\ 
%% \mbox{Assignment Stmt } \var := \aexpr & \rightarrow & \var := [\{\aexpr+1, \aexpr-1,\aexpr, 0 \}]\\ 
%% \mbox{Boolean Expr } \aexpr_0 ~ \bop ~  \aexpr_1 ~ & \rightarrow & \aexpr_0 ~ \sbop ~ \{\aexpr_1 + 1,\aexpr_1 - 1, 0 \} \\ 
%% & & \hspace*{-12mm}\mbox{where } \sbop = \{<, >, \leq, \geq, ==, \neq\}\\ 
%% \end{eqnarray*}
%% \end{minipage}
%% &
%% \begin{minipage}{3.5in}
%% \begin{eqnarray*}
%% \mbox{Function Params } f(\aexpr_1,\cdots,\aexpr_n) & \rightarrow  & f(\saexpr_1,\cdots,\saexpr_n)\\
%% & & \hspace*{-23mm}\mbox{where } \saexpr_i = \{\aexpr_i + 1, \aexpr_i - 1, \aexpr_i \}\\ 
%% \mbox{Base Case Inj } \sexpr & \rightarrow & \sexpr_{base};\sexpr\\
%% \mbox{Boolean Expr } \aexpr_0 ~ \bop ~  \aexpr_1 ~ & \rightarrow & \aexpr_0 ~ \sbop ~ \{\aexpr_1 + 1,\aexpr_1 - 1, 0 \} \\ 
%% & & \hspace*{-12mm}\mbox{where } \sbop = \{<, >, \leq, \geq, ==, \neq\}\\ 
%% \end{eqnarray*}
%% \end{minipage} \\
%% (a) & (b) \\
%% \end{tabular}
%% \caption{The transformation rules for (a) loop programs over arrays and (b) recursion programs}
%% \label{fig-lang-table}
%% \end{figure*}



==> related-work/intro.tex <==
\section{Introduction}

There has been a lot of recent interest in making education more accessible through information technology. Recently, for example, Sebastian Thurn and Peter Norving at Stanford made headlines when they allowed everyone in the world to register for their class and take it over the internet. One of the big bottlenecks in making this approach work, however, is the question of providing feedback to students, particularly when it comes to exams and assignments; in the case of the Stanford course, for example, 50,000 students turned in the first assignment\footnote{\label{NorvigAIClass}http://www.stanford.edu/group/knowledgebase/cgi-bin/2011/10/21/stanfords-online-engineering-classes-hugely-popular/}. Providing personalized human feedback for that many assignments is prohibitively expensive, so Norving and Thurn opted for not grading programming assignments; instead, students are assigned a grade by entering a few outputs from their program into a web form. The problem is that if their solution is not correct, the student does not get any feedback about what went wrong or how to fix it. The most a student gets in terms of feedback is a pointer to a video specifically recorded to help students who got the assignment wrong\footnotemark[\value{footnote}].

In this paper we show how---at least for introductory programming assignments---we can do much better than that. Specifically, this paper presents a new approach for automatically providing feedback describing exactly what was wrong with a student's solution to a programming problem. The approach leverages program synthesis technology to automatically determine minimal fixes to the student's program that will make it match the behavior of a reference solution written by the instructor. This technology makes it possible to provide students with precise feedback about what they did wrong, and provides a basis for assigning partial credit for incorrect assignments by giving a quantitative measure of the degree to which a solution was incorrect. 

\input{example1}


The problem of providing automatic feedback is closely related to the
problem of automated bug fixing, but it differs from it in three
important respects:
\begin{itemize}
\item \textbf{The correct solution is known.} An important challenge in automatic debugging is that there is no way to know
  whether a fix is addressing the root cause of a problem, or simply
  masking it and potentially introducing new errors. Usually the best
  one can do is check a candidate fix against a test suite or
a partial specification~\cite{rupakpldi11}. When grading on the other hand,
  the solution to the problem is known, and it is safe to assume that
  the teacher already wrote a correct reference implementation.

\item \textbf{Errors are predictable.} In a homework assignment,
  everyone is solving the same problem after having attended the same
  lectures, so errors tend to follow predictable patterns. This makes it possible to use a model-based
  debugging approach, where the potential fixes are guided by a
  model of the kinds of errors programmers make.

\item \textbf{Programs are small.} This is particularly true for
  introductory programming assignments, where students are learning
  basic programming constructs as well as simple algorithms like
  sorting. This makes the problem fundamentally different from the
  problem of debugging large-scale software.
\end{itemize}
These simplifying assumptions, however, introduces their own set of challenges. For example, while the problem specification is known, we cannot assume that teachers of introductory programming courses will write formal specifications, so the feedback tool needs to be able to reason about equivalence with a reference implementation. Also, in order to take advantage of the predictability of errors, the tool needs to provide a simple mechanism to describe classes of errors. And finally, while the codes are small, they can be expected to have more errors than production code, so techniques like the one suggested by ~\cite{rupakpldi11}, which attempt to correct bugs one path at a time will not work for many of these problems which require coordinated fixes in multiple places.

Our automated grading technique fulfills all of these requirements. The system can reason about the semantic equivalence of programs and reference implementations in a subset of C\#, so the teacher does not have to learn a new formalism to write specifications. The system also provides a \emph{correction} language that teachers can use to write an
\emph{error model}: a very high level description of potential
corrections to errors that students might make in the assignment. When
the system encounters an incorrect solution by a student, it
symbolically explores the space of all possible combinations of corrections allowed by the error model and finds a correct solution requiring a minimal set of corrections.

In order to evaluate our approach, we leveraged the \pexfun
website\footnote{Pex4Fun http://pex4fun.com}. \pexfun is a popular
website maintained by the Pex team at Microsoft Research as a way to
showcase their automated testing technology. The website allows people
to submit programming problems and puzzles, which are routinely solved
by people all over the world. When a user submits a candidate
solution, the site applies automated testing technology to find test
inputs for which a submission fails. The website records all solution
attempts by users, and distinguishes between attempts from different
users, so it is possible to use the website logs to observe how users
struggle to solve the programming problems and to see exactly what
errors they make even when given feedback in the form of input-output
pairs. While we have no way of knowing exactly who the users of the
website are (the logs are anonymized), it is safe to assume many of
them are beginner programmers given the kind of mistakes they make on
the programming problems, so we often refer to them as students or
beginners through the rest of the paper.

As part of our evaluation, we analyzed over a thousand solution attempts to problems including loops-over-arrays problems such as array reverse, recursion problems such as factorial, as well as more complex problems from Advanced Placement computer science exams\footnote{Advanced Placement Computer Science http://www.collegeboard.com/student/testing/ap/sub\_compscia.html}. We observe that \pexfun users tend to repeat similar mistakes when solving these problems and that our error models on average can correct over $70\%$ of submissions with small errors, \ie{} $70\%$ of those submissions that compiled with our tool and were not trivially incorrect, for example by being empty. We also show that the error models generalize well across different problems from the same category and that our technique scales well even for complex error models and larger programming assignments such as those found in AP examinations.


This paper makes the following key contributions:
\begin{itemize}
\item We show that the problem of automatically providing feedback for introductory programming assignments can be framed as a synthesis problem and successfully attacked using constraint-based synthesis technology.
\item We define a high-level language that instructors can use to provide correction rules to be used for automated grading. We also show that a small set of such rules is sufficient to correct hundreds of incorrect solutions produced by real beginner programmers.
\item We present a technique to compute minimum cost corrections
  to a student program based on the correction rules provided by an instructor.
\item We report the successful evaluation of our technique on over 1000 solution attempts by real beginner programmers on problems ranging from introductory programming problems to problems from AP level exams.
\end{itemize}


==> related-work/macros.tex <==
\newcommand{\impl}{\textsc{Imp}}
\newcommand{\implp}{\widetilde{\textsc{Imp}}}


%syntax and semantics macros
\renewcommand\t[1]{\texttt{#1}}
\newcommand\bnfas{\;:=\;}
\newcommand\bnfalt{\;|\;}
\newcommand\var{v}
\newcommand\expr{e}
\newcommand\fvar{f}
\newcommand\sem[1]{[\![#1]\!]}
\newcommand\state{\sigma}
\newcommand\emptystr{\epsilon}

%IMP language
\newcommand\prog{p}
\newcommand\aexpr{a}
\newcommand\bexpr{b}
\newcommand\sexpr{s}
\newcommand\intN{n}
\newcommand\op{op}
\newcommand\aop{op_\aexpr}
\newcommand\bop{op_\bexpr}
\newcommand\cop{op_c}
\newcommand\trueB{\t{true}}
\newcommand\falseB{\t{false}}
\newcommand\fs{\tilde{f}}

%IMP prime language
\newcommand\exprs{\tilde{\expr}}
\newcommand\saexpr{\tilde{\aexpr}}
\newcommand\sbexpr{\tilde{\bexpr}}
\newcommand\ssexpr{\tilde{\sexpr}}
\newcommand\saop{\widetilde{op}_a}
\newcommand\sbop{\widetilde{op}_b}
\newcommand\scop{\widetilde{op}_c}
\newcommand\svar{\tilde{\var}}
\newcommand\sintN{\tilde{\intN}}
\newcommand\schoose{\t{Choose}}
\newcommand\where{\;|\;}
\newcommand\choosevar{?}


\newcommand\csharp{\textsc{C\#}\xspace}
\newcommand\fuzzc{\widetilde{\textsc{C\#}}}
\newcommand {\Sk}{\textsc{Sketch}}
\newcommand{\fm}{\mathcal{F}}
\newcommand{\initF}{\textsc{InitF}}
\newcommand{\condF}{\textsc{CondF}}
\newcommand{\indF}{\textsc{IndF}}
\newcommand{\retF}{\textsc{RetF}}
\newcommand{\incF}{\textsc{IncF}}
\newcommand{\arithF}{\textsc{ArithF}}
\newcommand{\dash}{'}
\newcommand{\baseF}{\textsc{baseF}\xspace}

%transformExpr semantics
\newcommand{\transExpr}{\textsc{RewriteF}\xspace}
\newcommand{\matchE}{\t{Match}\xspace}
\newcommand{\subExpr}{\t{SubExprs}}
\newcommand{\replaceE}{\t{Replace}}
\newcommand{\tagged}{\t{Tagged}}
\newcommand{\varinscope}{\t{VarsInScope}}
\newcommand{\cost}{\t{cost}\xspace}
\newcommand{\hole}{h}
\newcommand{\sif}{\t{if}~}
\newcommand{\swhile}{\t{while}~}
\newcommand{\selse}{\t{else}~}
\newcommand{\sreturn}{\t{return}~}
\newcommand{\wexpr}{w}
\newcommand{\elseif}{\t{elif}~}

%translation to sketch
\newcommand\fuzzarithexpr{\t{FuzzArithExpr}}
\newcommand\fuzzboolexpr{\t{FuzzBoolExpr}}
\newcommand\fuzzstmtexpr{\t{FuzzStmtExpr}}
\newcommand\sh{\tilde{h}}
\newcommand\tmp{\t{tmp}}

\usepackage{listings}
\usepackage[T1]{fontenc}
\usepackage[scaled=0.8]{luximono}
\lstdefinelanguage{csh}{%
 morekeywords={%
  bool, true, false
     , public
     , class, static
     , int, while, for
     , return, implies
 },
 morecomment=[l]{//},
 otherkeywords={??},
 mathescape=true,
}
\lstset{numbers=left,numberblanklines=false, xleftmargin=.1in, ,numbersep=3pt, basicstyle=\tt,language=csh}
\newcommand{\C}[1]{\lstinline!#1!}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etal}{\textit{et al.}\@\xspace}
\newcommand{\eg}{\textit{e.g.}\@\xspace}
\newcommand{\ie}{\textit{i.e.}\@\xspace}

% References
%
%\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Property}

\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}

\newcommand{\corlabel}[1]{\label{cor:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}

\newcommand{\proplabel}[1]{\label{prop:#1}}
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\exlabel}[1]{\label{ex:#1}}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\problabel}[1]{\label{prob:#1}}
\newcommand{\probref}[1]{Problem~\ref{prob:#1}}
\newcommand{\obslabel}[1]{\label{obs:#1}}
\newcommand{\obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\alglabel}[1]{\label{alg:#1}}
\newcommand{\algref}[1]{Algorithm~\ref{alg:#1}}
%
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\shortsecref}[1]{\S\ref{sec:#1}}
\newcommand{\longsecref}[1]{Section~\ref{sec:#1}}
%
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\longfigref}[1]{Figure~\ref{fig:#1}}
\newcommand{\shortfigref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\eqqlabel}[1]{\label{eq:#1}}
\newcommand{\shorteqqref}[1]{\eqref{eq:#1}}
\newcommand{\mediumeqqref}[1]{Eq.~\eqref{eq:#1}}
\newcommand{\longeqqref}[1]{Equation~\eqref{eq:#1}}

% Determine type of references for particular document.
%
\newcommand{\secref}[1]{\longsecref{#1}}
\newcommand{\figref}[1]{\longfigref{#1}}
\newcommand{\eqqref}[1]{\longeqqref{#1}}

\newcommand{\pexfun}{\textsc{Pex4Fun}\xspace}
\newcommand{\funcF}{\textsc{FuncF}}
\newcommand{\basecF}{\textsc{BaseF}}



==> related-work/oldsection2.tex <==






\begin{figure*}
\begin{tabular}{|c|c|}
\hline
\begin{minipage}{3.4in}
\begin{lstlisting}
using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = a;
    for (int i=1; i<=b.Length/2; i++){
      int temp = b[i];  
      b[i] = b[b.Length-i];  
      b[b.Length-i] = temp;  
    }
    return b;
  }
}
\end{lstlisting}
\end{minipage}

&
\begin{minipage}{3.4in}
\begin{verbatim}
Fix 1: Decrement index i by 1 in lines 7 and 8.

Fix 2: Decrement index b.Length-i by 1 in lines 8 
       and 9, Change for loop initiation i to 0.
\end{verbatim}
\end{minipage}
\\\hline
\end{tabular}
\caption{Two possible fixes to fix the student's attempt on the left}
\figlabel{multiple-fix}
\end{figure*}

Our tool is able to provide direct feedback to the student about what went wrong with their program. 



\subsection{Why another metric?}

The traditional way to grade programs have been using test cases. The
instructors typically have a collection of test cases and the student
is awarded marks corresponding to the fraction of test cases that the
student's implementation successfully passes. It is not a very
satisfactory way of grading because of two reasons. First, a program
which is very close to the correct solution may fail all the test
cases whereas a program which is far from the desired solution may
pass many test cases (a collection of if statements for each test
case). The second reason is that test cases do not translate to good
feedback, especially for beginner
students. Figure~\ref{fig-log-diverge} shows the log of a student's
attempt for array reverse problem taken from pex4fun where the
feedback that the system provided to the student was in the form of
passing and failing test cases. It is quite interesting to see that
during the course of solving the problem, the student first came close
to the correct solution but then diverged away by fixing the wrong
part of solution.

Another way to grade programs is to perform syntactic matching of
student's solution with the teacher's reference solution. This can
lead to providing better feedback if the student solutions are of a
similar kind to the reference solution.  This grading scheme is very
specific to the refrence solution and we can not expect students to
write algorithms in a way exactly similar to what teacher has in
mind. Figure~\ref{fig-different-attempts} shows some of the student
solutions for array reverse problems. The student solution in (a) uses
a while loop with two pointers front and back and the student solution
in (b) uses a for loop with half traversal over the array, whereas the
teacher soultion does a single complete traversal over the array using
a for loop.



\subsection{Semantic grading with feedback}

In this paper, we present a framework for performing atuomated
semantic grading of student programs. Our framework assigns a
quantitative score to a student solution based on a closeness
metric. The closeness metric defines how many changes we need to
perform in the student solution to make it semantically equivalent to
the teacher reference solution. Figure~\ref{fig-feedback} shows the
score and feedback provided by our framework to the student solution
on the left.

It is not always possible to understand automatically what the student
has in mind. For example Figure~\ref{fig-multiple-fix} shows two
possible fixes to the student solution on the left. The first fix
suggests to decrement the array index \texttt{i} by $1$ in lines $7$
and $8$ corresponding to the case of missing the first array
element. Another fix might be to initialize the loop variable
\texttt{i} to $0$ and decrement the array indices $\texttt{b.Length}
-\texttt{i}$ by $1$ in lines $8$ and $9$. Our framework optimizes on
the mininum number of changes that are needed to be performed, but
also supports for providing multiple fixes if the student feels the
provided feedback does not correspond to the intended algorithm.





\begin{figure*}
\begin{tabular}{|c|c|c|}
\hline
\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length-1; i<a.Length-1; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
  }
}

\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length-1; i<a.Length-1; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
  }
}

\end{verbatim}
\end{minipage}
\\
6:28:50 AM
&
6:32:01 AM
&
6:32:32 AM
\\\hline

\hline
\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<=a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      Console.Writeline(i);
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      Console.WriteLine(i);
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}
\\
6:33:19 AM
&
6:33:55 AM
&
6:34:06 AM
\\\hline

\hline
\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i=<a.Length; i--)
    {
      Console.WriteLine(i);
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length-1];
    int count = 0;
    for(int i=a.Length-1; i<a.Length-1; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}
\\
6:34:56 AM
&
6:36:24 AM
&
6:37:39 AM
\\\hline

\hline
\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i>0; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i>=0; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<i.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}
\\
6:38:11 AM
&
6:38:44 AM
&
6:39:33 AM
\\\hline

\hline
\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length];
    int count = 1;
    for(int i=a.Length; i<a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
     
  }
}
\end{verbatim}
\end{minipage}

&

\begin{minipage}{2.2in}
\scriptsize
\begin{verbatim}

using System;

public class Program {
  public static int[] Puzzle(int[] a) {
    int[] b = new int[a.Length-1];
    int count = 0;
    for(int i=a.Length; i<a.Length; i--)
    {
      b[count] = a[i];
      count++;
    }
    return b;
  }
}
\end{verbatim}
\end{minipage}
\\
6:39:45 AM
&
6:40:27 AM
&
6:40:57 AM
\\\hline

\end{tabular}
\caption{Log of a student's attempts for array reverse problem}
\label{fig-log-diverge}
\end{figure*}




%% two column table example file
%% \begin{figure*}
%% \begin{tabular}{|c|c|}
%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length-1; i<a.Length-1; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }

%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:28:50 AM
%% &
%% 6:32:01 AM
%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length-1];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<=a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:32:32 AM
%% &
%% 6:33:19 AM

%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       Console.Writeline(i);
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       Console.WriteLine(i);
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }

%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:33:55 AM
%% &
%% 6:34:06 AM

%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i=<a.Length; i--)
%%     {
%%       Console.WriteLine(i);
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }

%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:34:56 AM
%% &
%% 6:36:24 AM

%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length-1];
%%     int count = 0;
%%     for(int i=a.Length-1; i<a.Length-1; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i>0; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:37:39 AM
%% &
%% 6:38:11 AM

%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i>=0; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<i.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:38:44 AM
%% &
%% 6:39:33 AM

%% \\\hline

%% \hline
%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{3.4in}
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 1;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\\hline
%% 6:39:45 AM
%% &
%% 6:40:27 AM

%% \\\hline

%% \end{tabular}
%% \end{figure*}



==> related-work/related.tex <==
\section{Related Work}

\subsection{AI based programming tutors}
There has been a lot of work done in the AI community for building
automated tutors for helping novice programmers learn programming by
providing feedback about semantic errors. These tutoring systems can
be categorized in two major classes: (i) systems that match student's
attempt with teacher's solution using some intermediate representation
of the implementations and (ii) systems that try to infer the student
intention (goals and plans) first and then match these intentions with
that of the teacher.

{\bf Code-based matching approaches:} LAURA~\cite{laura} converts
teacher's solution and student's attempt into a graph based
representation. It then compares them by heuristically applying
program transformations and reports mismatches as potential bugs. This
approach works well if the teacher's algorithm is exactly the same as
that of the student, but students typically solve the same problem
using many different algorithms as we have noted in our dataset as
well. TALUS~\cite{talus} matches a student's attempt with a collection
of teacher's algorithms. It first tries to recognize the algorithm
used in the student's attempt and then compares the attempt with the
recognized algorithm using symbolic evaluation on a set of cases. The
top-level expressions in the student's attempt are replaced
tentatively with expressions in the algorithm for generating
correction feedback. The problem with this approach is that the
enumeration of all possible algorithms (with its variants) for
covering all corrections is very large and tedious on part of the
teacher.

{\bf Intention-based matching approaches:} LISP tutor~\cite{lisptutor}
creates a model of the student goals and updates it dynamically as the
student makes edits. For incorrect edits, it provides suggestions
based on the teacher's model of inferred student intentions. The
drawback of this approach is that it forces students to write code in
a certain pre-defined structure and limits their freedom.
MENO-II~\cite{meno} parses student programs into a deep syntax tree
whose nodes are annotated with plan tags. This annotated tree is then
matched with the plans obtained from teacher's solution (provided in a
high level language PDL). PROUST~\cite{proust}, on the other hand,
uses a knowledge base of goals and their corresponding plans for
implementing them for each programming problem. It first tries to find
correspondence of these plans in the student's code and then performs
matching to find discrepancies. CHIRON~\cite{chiron} is its improved
version in which the goals and plans in the knowledge base are
organized in a hierarchical manner based on their generality and uses
machine learning techniques for plan identification in the student
code. These approaches require teacher to provide all possible plans a
student can use to solve the goals of a given problem and do not
perform well if the student's attempt uses a plan not present in the
knowledge base.

Our approach performs semantic equivalence of student's attempt and
teacher's solution based on an exhaustive bounded set of input-output
pairs and makes no assumptions on the algorithms or plans that
students can use for solving the problem. Moreover, our approach is
modular with respect to error models, as the teacher only needs to
provide local correction rules in a declarative manner and their
complex interactions are handled by the solver itself. We have
justified the advantages of our approach using analytical comparison;
we could have presented an experimental comparison as well, only if
their implementations were available.

\subsection{Automated Program Repair}

K$\ddot{o}$nighofer et. al.~\cite{prfmcad11} recently presented an
approach for automated error localization and correction of imperative
programs. They use model-based diagnosis to localize components that
need to be replaced and then use a template-based approach for
providing corrections using SMT reasoning. Their fault model only
considers the right hand side (RHS) of assignment statements as
replaceable components. The approaches in~\cite{JobstmannGB05,staber}
frame the problem of program repair as a game between an environment
that provides the inputs and a system that provides correct values for
the buggy expressions such that the specification is satisfied. It
isn't surprising that these approaches only support simple corrections
(e.g. correcting RHS side of expressions) in the fault model as they
aim to repair large programs with arbitrary errors. In our setting, we
exploit the fact that beginner student programs are small and we have
access to the dataset of previous student mistakes that we can use to
construct a \emph{concise and precise} fault model. This enables us to
model more sophisticated transformations such as introducing new
program statements, replacing LHS of assignments etc. in our error
model. Our approach also supports minimal cost changes to student's
programs where each error in the model is associated with a certain
cost, unlike the earlier mentioned approaches.

Mutation-based program repair~\cite{mutationicst} performs mutations
repeatedly to statements in a buggy program in order of their
suspiciousness until the program becomes correct. The problem with
this approach is that there is a large state space of mutants
(approximately of the order of $10^7$ in our case studies) and
explicitly enumerating them is infeasible. Our approach uses a
symbolic search for exploring correct solutions over this large set of
mutants. There are also some genetic programming approaches that
exploit redundancy present in some other part of the code for fixing
faults~\cite{arcuri,weimer}. These techniques are not applicable in
our setting as we do not have such redundancy present in small
introductory programming problems.

\subsection{Automated Debugging and Fault localization}

Techniques like Delta Debugging ~\cite{deltadebugging} and
QuickXplain~\cite{quickexplain} aim to simplify a failing test case
to a minimal test case that still exhibits the same failure. Our
approach can be complemented with these techniques to restrict the
application of rewrite rules to certain failing parts of the program
only. There are many algorithms for fault localization~\cite{fl1,fl2}
that use the difference between faulty and successful executions of
the system to identify potential faulty locations. Jose
et. al.~\cite{rupakpldi11} recently suggested an approach that uses a
MAX-SAT solver to satisfy maximum number of clauses in a formula
obtained from a failing test case to compute potential error
locations. These approaches, however, only localize faults for a
single failing test case and the suggested error location might not be
the desired error location, since we are looking for common error
locations that cause failure of multiple test cases. Moreover, these
techniques provide only a limited set of suggestions (if any) for
repairing these faults.

\subsection{Program Synthesis}

Program synthesis has been used recently for many applications such as
synthesis of efficient low-level code~\cite{solar2005bitstreaming,
  completefunctionalsynthesis}, bit-vector and graph
algorithms~\cite{sumitgraph, sumitbitvector}, snippets of excel
macros~\cite{excelpopl} and angelic
programming~\cite{angelicpopl}. The
\Sk~tool~\cite{solar2005bitstreaming,sketchthesis} takes a partial
program and a reference implementation as input and uses
constraint-based reasoning to synthesize a complete program that is
equivalent to the reference implementation. In general cases, the
template of the desired program as well as the reference specification
is unknown and puts an additional burden on the users to provide them;
in our case we use the student's solution as the template program and
teacher's solution as the reference implementation. A recent work by
Gulwani et. al.~\cite{sumitgeometry} also uses program synthesis
techniques for automatically synthesizing solutions to ruler/compass
based geometry construction problems. Their focus is primarily on
finding a solution to a given geometry problem whereas we aim to grade
and provide feedback on a given programming exercise solution. A
comprehensive survey on various program synthesis techniques and
different intention mechanisms for specification can be found
in~\cite{sumitsurvey}.


%% \subsection{Constraint-based Program Synthesis}

%% The idea of using a constraint-based approach for abstract
%% interpretation was previously introduced by Gulwani
%% \etal~\cite{GulwCBA}.  Recently, their group has used similar
%% techniques to synthesize invariants~\cite{GulwConstraintPredInf} and
%% even complete programs~\cite{SrivPts}. Some important distinctions
%% between their work and ours are the use of storyboards to capture
%% insights, as well as our path-based representation of the constraints
%% to support a very large and complex abstract domain.   The idea
%% of using a sketch to define the structure of the implementation was
%% adapted from the original work on sketch based
%% synthesis~\cite{pldi07-solar-etal}. The idea was originally applied
%% to the domain of bit-stream
%% manipulations~\cite{solar2005bitstreaming}, such as ciphers and
%% error correction codes, and has been applied more recently to
%% scientific programs~\cite{pldi07-solar-etal} and concurrent
%% data-structures~\cite{sketch08}.


%% \begin{figure*}
%% \begin{tabular}{|c|c|c|}
%% \hline
%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length-1; i<a.Length-1; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }

%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length-1; i<a.Length-1; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }

%% \end{verbatim}
%% \end{minipage}
%% \\
%% 6:28:50 AM
%% &
%% 6:32:01 AM
%% &
%% 6:32:32 AM
%% \\\hline

%% \hline
%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<=a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       Console.Writeline(i);
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       Console.WriteLine(i);
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\
%% 6:33:19 AM
%% &
%% 6:33:55 AM
%% &
%% 6:34:06 AM
%% \\\hline

%% \hline
%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i=<a.Length; i--)
%%     {
%%       Console.WriteLine(i);
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length-1];
%%     int count = 0;
%%     for(int i=a.Length-1; i<a.Length-1; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\
%% 6:34:56 AM
%% &
%% 6:36:24 AM
%% &
%% 6:37:39 AM
%% \\\hline

%% \hline
%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i>0; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i>=0; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<i.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\
%% 6:38:11 AM
%% &
%% 6:38:44 AM
%% &
%% 6:39:33 AM
%% \\\hline

%% \hline
%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length];
%%     int count = 1;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
     
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}

%% &

%% \begin{minipage}{2.2in}
%% \scriptsize
%% \begin{verbatim}

%% using System;

%% public class Program {
%%   public static int[] Puzzle(int[] a) {
%%     int[] b = new int[a.Length-1];
%%     int count = 0;
%%     for(int i=a.Length; i<a.Length; i--)
%%     {
%%       b[count] = a[i];
%%       count++;
%%     }
%%     return b;
%%   }
%% }
%% \end{verbatim}
%% \end{minipage}
%% \\
%% 6:39:45 AM
%% &
%% 6:40:27 AM
%% &
%% 6:40:57 AM
%% \\\hline

%% \end{tabular}
%% \caption{Log of a student's attempts for array reverse problem}
%% \label{fig-log-diverge}
%% \end{figure*}



==> related-work/technique.tex <==
\section{Algorithm}

From the student program and the fuzz model, create a family of programs close to the student solution.

Use constraint-based synthesis techniques to search for the closest
correct solution to the student solution.


==> technique.tex <==
\section{Algorithm}

From the student program and the fuzz model, create a family of programs close to the student solution.

Use constraint-based synthesis techniques to search for the closest
correct solution to the student solution.


==> weigthedimplp.tex <==
\section{Weighted $\implp$ programs}

A program in $\implp$ represents a set of $\impl$ programs and is
obtained by transforming an $\impl$ program using an error model. We
associate a cost metric $c$ (weight) with each $\impl$ program in the
set represented by $\implp$, where $c$ encodes the number of
modifications performed in the original program to obtain the
transformed program. This quantification allows us to solve for
finding correct programs that require minimum modifications
(i.e. minimum cost). \figref{fig-implp-cost} shows the recursive
algorithm to efficiently compute the cost associated with a
transformed program. For terminals in $\impl$ such as integers
($\intN$) and operators ($\op$), we associate a cost of $0$ if the
terminal in the transformed term is the same terminal as that in the
original term (where the original terminal is denoted by an underline
below it). If the transformed term contains some other terminal that
the terminal in the original term, we associate a cost of $1$ with
such a transformed term. For the set of expressions, if the
transformed expression is the same as the original expression
$\aexpr$, we associate a cost $c$ with the transformed expression and
a cost $c+1$ if it is different, where $c$ denotes the cost associated
with the expression $\aexpr$. The costs for other constructs in the
language are similarly computed recursively as shown in the figure.\\

\noindent{\bf Extension of cost metric:} We have presented a
simplified cost metric of associating cost $1$ with each
correction. The cost framework can easily be extended to account for
different costs associated with different corrections. This is usually
the case when instructors want to penalize students based on the kind
of mistake. For example, forgetting to add a base case in a recursion
problem might deserve more penalty than making a mistake in using the
conditional operator $<$ instead of $\leq$. The function of
\emph{adding} costs of sub-expressions to compute the cost of an
expression can also be generalized to other functions to cater for
different grading schemes.

%% \begin{figure}
%% \hspace*{-3mm}\begin{program}[style=tt,number=true]
%% \stab{1mm}\hspace*{-2mm}\underline{$\transExpr$}($\expr$: $\impl$, $\fm$: $\impl \rightarrow \implp$)\nonumber 
%% if $\matchE(\expr, L_1)$ then $\exprs = \exprs \cup \transSubExpr(R_1)$
%% if $\matchE(\expr, L_2)$ then $\exprs = \exprs \cup \transSubExpr(R_2)$
%% $\vdots$
%% $\exprs = \exprs \cup \{\expr\}$
%% $\t{return}~\exprs$
%% \end{program}
%% \end{figure}




%% \begin{figure*}
%% \begin{tabular}{c|c}
%% \begin{minipage}{3.5in}
%% \begin{eqnarray*}
%% \mbox{Arithmetic Expression } \aexpr & \bnfas & \intN \\
%%                          & \bnfalt & \var \\
%%                          & \bnfalt & \var[a]\\
%%                          & \bnfalt & \aexpr_0 ~ \aop ~ \aexpr_1\\
%%                           & \bnfalt & f(\aexpr_1, \cdots, \aexpr_n)\\
%% \mbox{Arithmetic Operator } \aop & \bnfas & + ~ \bnfalt ~ - ~ \bnfalt ~ \times\\
%% \mbox{Boolean Expression } \bexpr & \bnfas & \lnot ~ \bexpr\\
%%                           & \bnfalt & \aexpr_0 ~ \bop ~ \aexpr_1 \\
%%                           & \bnfalt & \bexpr_0 ~ \cop  ~ \bexpr_1\\
%% \mbox{Boolean Operator } \bop & \bnfas & == ~ \bnfalt ~ < ~ \bnfalt  ~ > ~ \bnfalt~ \leq ~ \bnfalt \geq\\
%% \mbox{Boolean Conjunction } \cop & \bnfas & \land ~ \bnfalt ~ \lor\\
%% \mbox{Statement Expression } \sexpr & \bnfas & \var := \aexpr \\
%%                            & \bnfalt & \sexpr_0;\sexpr_1\\
%%                            & \bnfalt & \t{if} ~ \bexpr ~ \t{then} ~ \sexpr_0 ~ \t{else} ~ \sexpr_1\\
%%                            & \bnfalt & \t{while} ~ \bexpr ~ \t{do} ~ \sexpr
%% \end{eqnarray*}
%% \end{minipage}
%% &
%% \begin{minipage}{3.5in}
%% \begin{eqnarray*}
%% \mbox{Arithmetic Expressions } \saexpr & \bnfas & \sintN \\
%%                          & \bnfalt & \svar \\
%%                          & \bnfalt & \svar[\saexpr]\\
%%                          & \bnfalt & \saexpr_0 ~ \saop ~ \saexpr_1\\
%%                           & \bnfalt & \tilde{f}(\saexpr_1, \cdots, \saexpr_n)\\
%% \mbox{Boolean Expressions } \sbexpr & \bnfas & \lnot ~ \sbexpr\\
%%                           & \bnfalt & \saexpr_0 ~ \sbop ~ \saexpr_1 \\
%%                           & \bnfalt & \sbexpr_0 ~ \scop  ~ \sbexpr_1\\
%% \mbox{Statement Expressions } \ssexpr & \bnfas & \svar := \saexpr \\
%%                            & \bnfalt & \ssexpr_0;\ssexpr_1\\
%%                            & \bnfalt & \t{if} ~ \sbexpr ~ \t{then} ~ \ssexpr_0 ~ \t{else} ~ \ssexpr_1\\
%%                            & \bnfalt & \t{while} ~ \sbexpr ~ \t{do} ~ \ssexpr
%% \end{eqnarray*}
%% \end{minipage} \\\\
%% $\impl$ & $\implp$ \\
%% \end{tabular}
%% \caption{The syntax for $\impl$ and $\implp$ languages}
%% \label{fig-lang-table}
%% \end{figure*}

\begin{figure*}
\begin{eqnarray*}
\sem{\{\intN\}} & = & \{(n,0)\}\\
\sem{\{\var\}} & = & \{(\var,0)\}\\
\sem{\{\underline{\op_0}, \cdots, \op_n\}} & = & \{(\op_i,1) \where 1 \leq i \leq n\} \cup \{(\op_0, 0)\}\\
\sem{\{\underline{\aexpr_0}, \cdots, \aexpr_n\}} & = & \{(\aexpr,~c+1) \where (\aexpr,c)\in\sem{\aexpr_i} \} \cup \sem{\aexpr_0}\\
\sem{\{\underline{\bexpr_0}, \cdots, \bexpr_n\}} & = & \{(\bexpr,~c+1) \where (\bexpr,c)\in\sem{\bexpr_i} \} \cup \sem{\bexpr_0}\\
\sem{\{\underline{\sexpr_0}, \cdots, \sexpr_n\}} & = & \{(\sexpr,~c+1) \where (\sexpr,c)\in\sem{\sexpr_i} \} \cup \sem{\sexpr_0}\\
\sem{\saexpr_0[\saexpr_1]} & = & \{(\aexpr_0[\aexpr_1],~c_0+c_1) \where (\aexpr_0,c_0)\in \sem{\saexpr_0}, (\aexpr_1,c_1) \in \sem{\saexpr_1} \}\\
\sem{?\var} & = & \{(\var_1,1) \where \var_1 \in \varinscope(\var), \var_1 \neq \var \} ~ \cup \sem{\var}\\
\sem{ \fs(\saexpr_1, \cdots, \saexpr_n} & = & \{(f(\aexpr_1,\cdots,\aexpr_n),~c_f+c_1\cdots+c_n) \where (f,c_f)\in\sem{\fs}, (\aexpr_i,c_i) \in \sem{\saexpr_i} \}\\
\sem{\saexpr_0 ~ \saop ~ \saexpr_1} & = & \{(\aexpr_0 ~ \aop ~ \aexpr_1, ~c_0+c_a+c_1) \where (\aexpr_0,c_0)\in\sem{\saexpr_0}, (\aop,c_a)\in\sem{\saop}, (\aexpr_1,c_1)\in\sem{\saexpr_1} \}\\
\sem{\saexpr_0 ~ \sbop ~ \saexpr_1} & = & \{(\aexpr_0 ~ \bop ~ \aexpr_1, ~c_0+c_b+c_1) \where (\aexpr_0,c_0)\in\sem{\saexpr_0}, (\bop,c_b)\in\sem{\sbop}, (\aexpr_1,c_1)\in\sem{\saexpr_1} \}\\
\sem{\sbexpr_0 ~ \scop ~ \sbexpr_1} & = & \{(\bexpr_0 ~ \cop ~ \bexpr_1, ~c_0+c_c+c_1) \where (\bexpr_0,c_0)\in\sem{\sbexpr_0}, (\cop,c_c)\in\sem{\scop}, (\bexpr_1,c_1)\in\sem{\sbexpr_1} \}\\
\sem{\svar := \saexpr} & = &  \{(\var := \aexpr, ~c_0 + c_1) \where (\var,c_0) \in \sem{\svar}, (\aexpr,c_1) \in \sem{\saexpr}\}\\
\sem{\ssexpr_0;\ssexpr_1} & = & \{ (\sexpr_0;\sexpr_1, ~c_0+c_1) \where (\sexpr_0,c_0) \in \sem{\ssexpr_0}, (\sexpr_1,c_1) \in \sem{\ssexpr_1}\}\\
\sem{\t{if} ~ \sbexpr ~ \t{then} ~ \ssexpr_0 ~ \t{else} ~ \ssexpr_1} & = & \{(\t{if} ~ \bexpr ~ \t{then} ~ \sexpr_0 ~ \t{else} ~ \sexpr_1, ~c_b+c_0+c_1) \where (\bexpr,c_b) \in \sem{\sbexpr}, (\sexpr_0,c_0) \in \sem{\ssexpr_0}, (\sexpr_1,c_1) \in \sem{\ssexpr_1}\}\\
\sem{\t{while} ~ \sbexpr ~ \t{do} ~ \ssexpr} & = & \{(\t{while} ~ \bexpr ~ \t{do} ~ \sexpr, ~ c_b + c_s) \where (\bexpr,c_b) \in \sem{\sbexpr}, (\sexpr,c_s) \in \sem{\ssexpr}\}\\ 
\sem{\t{return} ~ \saexpr} & = & \{(\t{return} ~ \aexpr, ~ c) \where (\aexpr,c) \in \sem{\aexpr}\}\\ 
\end{eqnarray*}
\caption{The translation of a program in $\implp$ to a set of programs in $\impl$, each associated with a cost $c$}
\figlabel{fig-implp-cost}
\end{figure*}

%% \begin{figure*}
%% \begin{center}
%%   \begin{tabular}{c c c}
%% \inference{t_1 \rightarrow_R t_2}{t_1 \rightarrow^{*}_R t_2}
%% &
%% \inference{t_1 \rightarrow^{*}_R t_3 & t_3 \rightarrow^{*}_R t_2}{t_1 \rightarrow^{*}_R t_2}
%% &
%% \inference{t_1 \rightarrow^{*}_R t'_1 ~~~~\cdots ~~~~ t_n \rightarrow^{*}_R t'_n}{c(t_1,\cdots,t_n) \rightarrow^{*}_R c(t'_1, \cdots, t'_n)}

%% \end{tabular}
%% \end{center}
%% \caption{Semantics for term rewriting rules}
%% \end{figure*}

%% \begin{figure*}
%% \begin{center}
%% \begin{tabular}{c c c}
%% \inference{t_1 \rightarrow^{i}_R t'_1 ~~~~\cdots ~~~~ t_n \rightarrow^{i}_R t'_n ~~~~ c(t'_1,\cdots,t'_n) \rightarrow^{r}_R t}{c(t_1,\cdots,t_n) \rightarrow^{i}_R t}
%% &
%% \inference{t_1 \rightarrow_R t_2 ~~~~ t_2 \rightarrow^{i}_R t_3}{t_1 \rightarrow^{r}_R t_3}
%% &
%% \inference{\lnot \exists t_2 : t_1 \rightarrow_R t_2 }{t_1 \rightarrow^{r}_R t_1}
%% \end{tabular}
%% \end{center}
%% \caption{Semantics for Innermost term rewriting strategy}
%% \end{figure*}

%% \begin{figure*}
%% \begin{tabular}{c|c}
%% \begin{minipage}{3.5in}
%% \begin{eqnarray*}
%% \mbox{Array Indexes } \var[\aexpr] & \rightarrow & \var[\{\aexpr+1, \aexpr-1,\aexpr \}]\\ 
%% \mbox{Assignment Stmt } \var := \aexpr & \rightarrow & \var := [\{\aexpr+1, \aexpr-1,\aexpr, 0 \}]\\ 
%% \mbox{Boolean Expr } \aexpr_0 ~ \bop ~  \aexpr_1 ~ & \rightarrow & \aexpr_0 ~ \sbop ~ \{\aexpr_1 + 1,\aexpr_1 - 1, 0 \} \\ 
%% & & \hspace*{-12mm}\mbox{where } \sbop = \{<, >, \leq, \geq, ==, \neq\}\\ 
%% \end{eqnarray*}
%% \end{minipage}
%% &
%% \begin{minipage}{3.5in}
%% \begin{eqnarray*}
%% \mbox{Function Params } f(\aexpr_1,\cdots,\aexpr_n) & \rightarrow  & f(\saexpr_1,\cdots,\saexpr_n)\\
%% & & \hspace*{-23mm}\mbox{where } \saexpr_i = \{\aexpr_i + 1, \aexpr_i - 1, \aexpr_i \}\\ 
%% \mbox{Base Case Inj } \sexpr & \rightarrow & \sexpr_{base};\sexpr\\
%% \mbox{Boolean Expr } \aexpr_0 ~ \bop ~  \aexpr_1 ~ & \rightarrow & \aexpr_0 ~ \sbop ~ \{\aexpr_1 + 1,\aexpr_1 - 1, 0 \} \\ 
%% & & \hspace*{-12mm}\mbox{where } \sbop = \{<, >, \leq, \geq, ==, \neq\}\\ 
%% \end{eqnarray*}
%% \end{minipage} \\
%% (a) & (b) \\
%% \end{tabular}
%% \caption{The transformation rules for (a) loop programs over arrays and (b) recursion programs}
%% \label{fig-lang-table}
%% \end{figure*}


